ShAPO: Implicit Representations for Multi-Object Shape, Appearance, and Pose Optimization

Our method studies the complex task of object-centric 3D understanding from a single RGB-D observation. As it is an ill-posed problem, existing methods suffer from low performance for both 3D shape and 6D pose and size estimation in complex multi-object scenarios with occlusions. We present ShAPO, a method for joint multi-object detection, 3D textured reconstruction, 6D object pose and size estimation. Key to ShAPO is a single-shot pipeline to regress shape, appearance and pose latent codes along with the masks of each object instance, which is then further refined in a sparse-to-dense fashion. A novel disentangled shape and appearance database of priors is first learned to embed objects in their respective shape and appearance space. We also propose a novel, octree-based differentiable optimization step, allowing us to further improve object shape, pose and appearance simultaneously under the learned latent space, in an analysis-by-synthesis fashion. Our novel joint implicit textured object representation allows us to accurately identify and reconstruct novel unseen objects without having access to their 3D meshes. Through extensive experiments, we show that our method, trained on simulated indoor scenes, accurately regresses the shape, appearance and pose of novel objects in the real-world with minimal fine-tuning. Our method significantly out-performs all baselines on the NOCS dataset with an 8% absolute improvement in mAP for 6D pose estimation. Project page: https://zubair-irshad.github.io/projects/ShAPO.html

==> tables/ablation.tex <==
\setlength{\tabcolsep}{16pt}
\begin{table*}[t]
\centering
\large
\renewcommand{\arraystretch}{1.3}
\caption{\textbf{Ablation Study of Different LoDs on Downstream task of 3D object detection and 6D pose estimation}: Study of the Proposed CenterSnap method on NOCS Real-test set to investigate the impact of different components i.e. Input, Shape, Training Regime~(TR) and Depth-Auxiliary loss~(D-Aux) on performance. C indicates Camera-train, R indicates Real-train and RF indicates Real-train with finetuning. 3D shape reconstruction evaluated with \textbf{CD} ($10^{-2}$). $*$ denotes the method does not evaluate size and scale and so has no IOU metric.}
% \zk{For ablation I would move (3) to second-to-last. Otherwise it's confusing what to get out of it (it seems C+RF is the dominant factor).
% Maybe also same for depth (2) as well. Otherwise it looks like going from D-> RGBD hurts performance}}
% \zk{Need arrows for higher/lower being better for each metric. You never mention this for lesser known ones such as CD, and it's not really clear (seems to be all over the place in ablation?)}}
% \zk{I think this is copied?}\zk{I assume below results aren't done yet? For example last three rows are the same results?}}
\label{tab:ablation}
\resizebox{1.0\textwidth}{!}{%
\begin{tabular}{c@{\hskip 0.1in}lccccccccc} \\
\toprule
& & & & \multicolumn{6}{c}{\textbf{Metrics}} \\ 
\cmidrule(r{0.05in}){6-6}
\cmidrule(r{0.05in}){7-10}

& & & & & \textbf{3D Shape} & \multicolumn{4}{c}{\textbf{6D Pose}} \\ 
% \cmidrule(){5-9}
\cmidrule(r{0.05in}){6-6}
\cmidrule(r{0.05in}){7-10}
 {\textbf{\#}} & \text{Shape Representation} &\text{LoD} &\text{Sparse(ICP)} & Dense(DR)&\textbf{CD}~$\downarrow$ & \textbf{IOU25}~$\uparrow$ & \textbf{IOU50}~$\uparrow$ &\textbf{5\textdegree \SI{10}{\cm}}~$\uparrow$ & \textbf{10\textdegree \SI{10}{\cm}}~$\uparrow$  \\

\midrule
 1 &PointCloud& - & C & \checkmark & 0.19 & 28.4 & 27.0 & 14.2 &48.2 \\
 2 &PointCloud& - & C+R & \checkmark & 0.19 & 41.5 & 40.1 & 27.1 & 58.2\\
 3 &Implicit& &LoD2 & \checkmark & --- & --- & --- & 13.8 & 50.2 \\
 4 & Implicit & LoD3 & \checkmark & \checkmark & 0.20 & 63.7 & 31.5 & 8.30 & 30.1\\
 5 &Implicit& LoD4 & C+RF & \checkmark & 0.15 & 74.2 & 66.7 & 30.2 & 63.2  \\
 6 &Implicit&LoD5  & C+RF&  & 0.17 & 82.3 & 78.3 & 30.8 &68.3 \\
 7 &Implicit& LoD6 & C+RF & \checkmark & 0.15 & 83.5 & 80.2 & 31.6 &70.9 \\
\bottomrule
\end{tabular}}
% \vspace{-1mm}
% \vspace{-0.15cm}
\end{table*}

% \setlength{\tabcolsep}{16pt}
% \begin{table*}[t]
%     \centering
%     \renewcommand{\arraystretch}{1.3}
%     \caption{
%     \textbf{Ablations of Different LoDs on of 3D object detection and 6D pose estimation on NOCS}~\cite{wang2019normalized}: Comparison with strong baselines. Best results are highlighted in \textbf{bold}. $*$ denotes the method does not evaluate size and scale hence does not report IOU metric. For a fair comparison with other approaches, we report the per-class metrics using nocs-level class predictions. Note that the comparison results are either fair re-evaluations from the author's provided best checkpoints or reported from the original paper.
%     }
%     \label{ablation_table}
%     \vspace{+0.15cm}
%     \resizebox{1.0\textwidth}{!}{
%     \begin{tabular}{clcccccc}
%         \toprule
%         & & \multicolumn{6}{c}{\textbf{REAL275}} \\ 
%         \cmidrule(r{0.1in}){3-8}
%         & {Method} & \textbf{IOU25} & \textbf{IOU50} & \textbf{5\textdegree \SI{5}{\cm}} & \textbf{5\textdegree \SI{10}{\cm}}& \textbf{10\textdegree \SI{5}{\cm}} & \textbf{10\textdegree \SI{10}{\cm}}\\
%         \cmidrule(r{0.1in}){2-2}
%         \cmidrule(r{0.1in}){3-8}
%         1 & {NOCS~\cite{wang2019normalized}}       & \textbf{84.8} & 78.0 & 10.0 & 9.8 & 25.2 & 25.8\\
%         2 & {Synthesis$^{*}$~\cite{chen2020category}} & - & - &  0.9 & 1.4 & 2.4 & 5.5 \\

%         3 & {Metric Scale~\cite{lee2021category}} & 81.6 & 68.1 & 5.3 & 5.5 & 24.7 & 26.5 \\
%         4 & {ShapePrior~\cite{tian2020shape}} &	81.2& 77.3	&	21.4	&21.4&	54.1&	54.1\\
%         5 & {CASS~\cite{chen2020learning}} & 84.2 & 77.7 &  23.5 & 23.8 & 58.0 & 58.3\\
%         6 & {CenterSnap}  &	80.2 & 27.2 &	29.2 & 58.8 &	64.4 \\
%     7 & {CenterSnap-R} & 83.5 &	\textbf{80.2} & \textbf{29.1} &	\textbf{31.6} & \textbf{64.3} &	\textbf{70.9} \\
%       \midrule
%     8 & {\textbf{Genie (Ours)}} &	\textbf{85.3} &	\textbf{83.2} & \textbf{32.0} &	\textbf{35.2} & \textbf{67.1} &	\textbf{74.1} \\
      
%         \bottomrule
%     \end{tabular}
%     }
%     % \vspace{-2mm}
% \end{table*}

==> tables/prior_works_related.tex <==
\setlength{\tabcolsep}{8pt}
\resizebox{1\linewidth}{!}{
\begin{tabular}{@{}lccccccc@{}}
\toprule
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}} 
Deep\\ SDF~\cite{park2019deepsdf}\end{tabular}}& FroDO~\cite{runz2020frodo}& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}} Holistic\\3D~\cite{zhang2021holistic}\end{tabular}}   & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}} Center\\Snap~\cite{irshad2022centersnap}\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}} Shape\\Prior~\cite{tian2020shape}\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}  \\\titleShort{} \\ (\textbf{Ours})\end{tabular}}\\ 
\midrule 
Object\\ Pose &     \xmark  &  \checkmark  & \checkmark & \checkmark  & \checkmark & \checkmark    \\
\cmidrule{2-7} 
End-to-End \\(Detection \& Reconstruction) & \xmark & \checkmark & \checkmark & \checkmark & \xmark & \checkmark\\
\cmidrule{2-7} 
Disentangled \\shape and texture & \xmark  & \xmark & \xmark & \xmark  & \xmark & \checkmark \\
\cmidrule{2-7} 
Shape\\ Representation & Implicit & Implicit/Points & Implicit & Points & Points & Implicit \\ %\midrule
\cmidrule{2-7} 
Sparse \& Dense \\optimizaiton & \checkmark & \xmark & \xmark & \xmark & \checkmark & \checkmark \\ %\midrule

\bottomrule
\\
\end{tabular}
}

% \begin{table*}[t]
%     \scriptsize
%     \centering
%     \renewcommand{\arraystretch}{1.3}
%     \caption{
%     \textbf{Comparison between our proposed Genie method and prior works} on object-centric 3D scene understanding.
%     }
%     \label{comparison_table}
%     % \vspace{+0.15cm}
%     \resizebox{1.0\textwidth}{!}{
%     \begin{tabular}{clcccccc}
%         \toprule
%         &  & \textbf{IOU25} & \textbf{IOU50} & \textbf{5\textdegree \SI{5}{\cm}} & \textbf{5\textdegree \SI{10}{\cm}} & \textbf{10\textdegree \SI{5}{\cm}} & \textbf{10\textdegree \SI{10}{\cm}}\\
%         \cmidrule(r{0.1in}){2-2}
%         \cmidrule(r{0.1in}){3-8}
%         1 & {Object Pose}      &  91.1& 83.9 & 40.9  & 38.6 & 64.6 & 65.1 \\
%         2 & {Disentangled shape\\ and texture} &  - & - & -  &- & - & -\\

%         3 & {Metric Scale~\cite{lee2021category}}      &  \textbf{93.8}& 90.7 & 20.2  & 28.2 & 55.4 & 58.9  \\
%         4 & {ShapePrior~\cite{tian2020shape}} &81.6	&72.4&	59.0&	59.6&  81.0 &  81.3\\
%         5 & {CASS~\cite{chen2020learning}} & - & - & - & - & - & \\
%         6 & {CenterSnap} & 93.2&	92.3&	63.0	& 69.5 &	79.5 & 87.9 \\
%         \bottomrule
%     \end{tabular}
%     }
%     % \vspace{-2mm}
% \end{table*}
%  \resizebox{1\linewidth}{!}{
% \begin{tabular}{SSSSSSSS} \toprule
%      & & {DeepSDF~\cite{park2019deepsdf}} & {FroDO~\cite{runz2020frodo}} & {Holistic3D~\cite{zhang2021holistic}} & {CenterSnap~\cite{irshad2022centersnap}} &{ShapePrior~\cite{tian2020shape}} & {Genie(\textbf(Ours))} \\ \midrule
%     1 & {Object Pose}& \checkmark  &  \checkmark  & \xmark & \checkmark  & \checkmark  & \\
%     2 &{Disentangled shape and texture} & 3D  & 2D & 2D & 2D  & 2D &       \\
%     3 & & 1.826  & -0.363 & 1.826  & 0.159 & 0.119 & 168.5 \\
%     4 & & 0.993  & -0.429 & 0.993  & 0.086 & 0.08  & 25.6 \\ \bottomrule
% \end{tabular}}

